KAM-renormalization and Herman rings for 2D maps

In this note, we extend the renormalization horseshoe we have recently constructed with N. Goncharuk for analytic diffeomorphisms of the circle to their small two-dimensional perturbations. As one consequence, Herman rings with rotation numbers of bounded type survive on a codimension one set of parameters under small two-dimensional perturbations.

==> renorm.tex <==
%!TEX root = main.tex
\medskip
\noindent

\section{Renormalization for  pairs of two-dimensional dissipative maps}\label{sec:RenACM}
This section contains a summary of the extention of the renormalization operator from the space $\cB(Z,W)$ of almost commuting pairs to an appropriately defined space of two-dimensional maps. The details of the procedure can be found in \cite{GaYa3}.

Let $\Omega, \Gamma$ be  domains in $\CC^2$. We denote $O(\Omega,\Gamma)$ the Banach space of bounded analytic functions 
$F=(F_1(x,y),F_2(x,y))$  from $\Omega$ and $\Gamma$ respectively to $\CC^2$ equipped with the norm
\begin{equation}
\label{eq:unormm}\| F\|= \frac{1}{2} \left(   \sup_{(x,y) \in \Omega}|F_1(x,y)|+  \sup_{(x,y)\in \Gamma} |F_2(x,y) | \right).
\end{equation}
 We let $O(\Omega,\Gamma,\delta)$ stand for the $\delta$-ball around the origin in this Banach space. 


In what follows, we fix $W$, $Z$, $\tl Z$, and $\tl W$ as in ({\bf H}), and $R>0$ such that $\DD_R \subset Z \cap W$, and let 
$\Omega=Z \times \DD_R$, $\Gamma=W \times \DD_R$.
We select $\hat Z$ and $\hat W$ so that
$$Z \Subset \hat Z \Subset \tl Z,\; W \Subset \hat W \Subset \tl W.$$
We define an isometric embedding $\iota$ of the space $\cH(Z,W)$ into $O(\Omega,\Gamma)$ which send the pair $\zeta=(\eta,\xi)$ to
the  pair of functions $\iota(\zeta)$:
\begin{equation}
\label{eq:embed}
\left(\left(x \atop  y\right)\mapsto \left(\eta(x) \atop \eta(x) \right), 
\left(x \atop  y\right)\mapsto \left(\xi(x) \atop \xi(x) \right)   \right).
\end{equation}


Let $\cU$ be an open neighborhood of $\zeta_\lambda$ as in ({\bf H}) in $\cC(Z,W)$, and let $Q$ be a neighborhood of $0$ in $\CC$.
We will consider an open subset of  $O(\Omega,\Gamma)$ of pairs of maps of the form
\begin{eqnarray}
\label{eq:A} A(x,y)&=&(a(x,y),h(x,y))=(a_y(x),h_y(x)),\\
\label{eq:B} B(x,y)&=&(b(x,y),g(x,y))=(b_y(x),g_y(x)), 
\end{eqnarray}
such that
\begin{itemize}
\item[1)] the pair $(a(x,y),b(x,y))$ is in a $\delta$-neighborhood  of  $\cU$ in $O(\Omega,\Gamma)$,
\item[2)]  $(h,g) \in O(\Omega,\Gamma)$ are such that  $|\partial_x h(x,0)|>0$ and  $|\partial_x g(x,0)|>0$ whenever $x \notin \bar Q$,  and 
$$(h(x,y)-h(x,0),g(x,y)-g(x,0)) \in O(\Omega,\Gamma,\delta).$$ 
\end{itemize}
This open subset of $O(\Omega,\Gamma)$ will be denoted $\cA(\cU,Q,\delta)$ for brevity.

We say that a pair $(A,B)$ is a pre-renormalization of a map $H$:
$$(A,B)=p\cR^nH$$ if 
$$A=H^{q_n},\;B=H^{q_{n+1}}\text{ for some }n\geq 0.$$


%Given a pair $\Sigma=(A,B)$ as in $(\ref{eq:A})-(\ref{eq:B})$ we set 
%$$\cL \Sigma \equiv (a(x,0),b(x,0)).$$



\subsection{Defining renormalization: coordinate transformations}

Let $(\eta,\xi) \in \cB(Z,W)$ be $n\geq 2$ times renormalizable,  and consider its $n$-th pre-renormalization written as
$$p \cR^n\zeta=\left( \zeta^{\bar s_n}, \zeta^{\bar t_n } \right).$$
Let $\bar s_n$ be given by $(a_1,b_1,a_2,b_2,\ldots,a_{m_n},0)$ (recall Lemma~\ref{multi1}).
We denote 
\begin{eqnarray}
\nonumber \hat s_n&=&\left\{ (a_1,b_1,a_2,b_2,\ldots,a_{m_n}-2,0), \ a_{m_n} \ge 2  \atop (a_1,b_1,a_2,b_2,\ldots,0,0,0), \ a_{m_n}=1 \right. ,\\
\nonumber \phi_0(x)&=&\left\{ \eta^2, \ a_{m_n} \ge 2  \atop \eta \circ \xi, \ a_{m_n}=1 \right. .
\end{eqnarray}
Define $\hat t_{n}$ in an identical way to $\hat s_{n}$ (see Lemma~\ref{multi1}). Then $p \cR^n\zeta$ can be written as
$$ p \cR^n\zeta=\phi_0 \circ  \left(\zeta^{\h s_n}, \zeta^{\h t_n } \right).$$
%%
 For a  sufficiently large $n$, the function $\eta^{-1}$ is a diffeomorphism of the neighborhood $\alpha_n (Z \cup W)$, and one can define the $n$-th pre-renormalization of $\zeta$ in $\eta^{-1}(\alpha_n (Z \cup W))$ as 
$$
\h p \cR^n\zeta=\left(\eta^{-1} \circ  \zeta^{\bar s_n} \circ \eta, \eta^{-1} \circ \zeta^{\bar t_n } \circ \eta \right)=\left( f \circ   \zeta^{\h s_n} \circ \eta, f \circ \zeta^{\h t_n } \circ \eta \right),
$$
where $f=\eta$ if $a_n \ge 2$ and $f=\xi$ if $a_n=1$.


Next, suppose that $\Sigma=(A,B)$ lies in $\cA(\cU,Q,\delta)$ with $\cU$ and $\delta$ sufficiently small, so that 
the following pre-renormalization  is defined in a neighborhood of $\eta^{-1}(\alpha_n (Z \cup W))\times \{ 0\}$:
$$\h p \cR^n \Sigma = \left(F \circ \Sigma^{\h s_n} \circ A, F \circ \Sigma^{\h t_n} \circ A \right),$$
where $F=A$ if $a_n \ge 2$ and $F=B$ if $a_n=1$.


We will denote $$\pi_1(x,y)=x\text{ and }\pi_2(x,y)=y.$$



Set
$$\phi_y(x)=\phi(x,y) :=\left\{ \pi_1 A^2(x,y), \ a_n \ge 2  \atop \pi_1 A \circ B(x,y), \ a_n=1 \right.$$

For sufficiently small $\delta$, the map $\phi_z$ is close to $\phi_0$ and is a diffeomorphism of a neighborhood of $\pi_1 \Sigma^{\h s_n}(\alpha_n(Z),0) \approx \zeta^{\h s_n}(\alpha_n (Z))$ for all $z \in \DD_R$ for some  $R=R(\delta)>0$.  Similarly, $g_z$ is a diffemorphism of  a neighborhood of $\pi_1  \Sigma^{\h s_n}(\alpha_n (Z),0)$ for all $z \in \DD_R$ for some $R=R(\delta)>0$.

Furthermore, set
$$q_z(x) \equiv q(x,z)=\pi_2 F(x,z)= \left\{ h_z(x), \ a_n \ge 2  \atop g_z(x), \ a_n=1 \right.$$
According to our definition of the class  $\cA(\cU,Q,\delta)$, this is a diffeomorphism outside a neighborhood of zero. Also, set
\begin{equation}
\nonumber w_z(x) \equiv w(x,z) := q_{z}\left(\phi_{z}^{-1}( x) \right),
\end{equation} 
a diffeomorphism of a neighborhood of   $\pi_1 \phi_z \circ \Sigma^{\h s_n}(\alpha_n (Z),0)$ in $\CC^2$ onto its image for all $z \in \DD_R$ for some  $R=R(\delta)>0$.  Notice, that $\partial_z  w_z(x)$ and $\partial_z w^{-1}_z(x)$ are functions whose uniform norms are $O(\delta)$.

\noindent
Define the following transformation:
\begin{equation}\label{eq:Htransform}
H_{\Sigma}(x,y) = (a_y(x),w_{q_0^{-1}(y)}^{-1}(y)),
\end{equation}
This transformation is $\delta$-close to $\left(\eta(x),\phi_0(q_0^{-1}(y)) \right)$ in $O(\Omega,\Gamma)$, and therefore, for small $\delta$,  is a diffieomorphism of a neighborhood of $\pi_1  F \circ \Sigma^{\h s_n}(\alpha_n (Z),0) \approx f(\zeta^{\h s_n}(\alpha_n (Z)))$ onto its image.  In particular, 
\begin{equation}
\label{eq:AHinv} A \circ H_{\Sigma}^{-1}(x,y)=(x,h(\eta^{-1}(x),y))+O(\delta).
\end{equation}

We use $H_{\Sigma}(x,y)$ to pull back $\hat p \cR^n \Sigma$ to a neighborhood of definition of the $n$-th pre-renormalization of a pair $(\eta,\xi)$ - that is, a neighborhood of  $\alpha_n (Z \cup W)$ in $\CC^2$:
$$p \cR^n \Sigma=(\bar A, \bar B) = H_{\Sigma}\circ F \circ \left( \Sigma^{\h s_n},  \Sigma^{\h t_n} \right) \circ A \circ H_{\Sigma}^{-1}(x,y).$$




The following has been proved in \cite{GaYa2}.
\begin{lem}
\label{lem-preren}
There exists an $n \in \NN$, and a choice of $\cU$, $Q$, $\delta_0$ and $C>0$ such that the following holds. For every $\delta<\delta_0$ and every $\Sigma\in\cA(\cU,Q,\delta)$ the pair $p\cR^n\Sigma$ is defined, lies in $O(\hat\Omega,\hat\Gamma)$, $\hat \Omega= \hat Z \times \DD_R$,  $\hat \Gamma= \hat W \times \DD_R$, and 
$$\dist(p \cR^n \Sigma, \iota(\cH(\alpha_n(\hat Z),\alpha_n(\hat W))))<{C \delta (\|  \pi_1 \Sigma-\pi_2 \Sigma\|+\delta   )}.$$
\end{lem}

Let us write
\begin{equation}
\bar{A}(x,y)=\left( { \bar \eta_1(x)+\bar \tau_1(x,y) \atop   \bar \eta_2(x)+\bar \tau_2(x,y) } \right),
\end{equation}
where 
$$\bar \eta_1(x) \equiv \pi_1 \bar{A}(x,0), \quad  \bar \eta_2(x) \equiv \pi_2 \bar{A}(x,0)$$
are $O({ \delta \|  \pi_1 \Sigma-\pi_2 \Sigma\|+\delta^{2}   })$-close to each other, and both are $\delta$-close to $\pi_\eta p \cR^n \zeta=\zeta^{\bar s_n}$, where  $\pi_\eta$ and $\pi_\xi$ are the projections on, correspondingly, the first and the second map in a pair, and 
$$\bar \tau_1(x,y) \equiv  \pi_1 \bar{A}(x,y)- \pi_1 \bar{A}(x,0), \quad \bar \tau_2(x,y)= \pi_2 \bar{A}(x,y)- \pi_2 \bar{A}(x,0),$$
are functions whose norms are $O(\delta^2)$. Similarly,
$$
\nonumber \bar{B}(x,y)=\left( { \bar \xi_1(x)+\bar \pi_1x,y) \atop   \bar \xi_2(x)+\bar \pi_2(x,y) } \right),
$$
where
$$\bar \xi_1(x) \equiv \pi_1 \bar{B}(x,0), \quad  \bar \xi_2(x) \equiv \pi_2 \bar{B}(x,0)$$
are $O({\delta \|  \pi_1 \Sigma-\pi_2 \Sigma\|+\delta^{2}   })$-close to each other, and both are $\delta$-close to $\pi_\xi p \cR^n \zeta=\zeta^{\bar t_n}$, and 
$$\bar \pi_1(x,y) \equiv  \pi_1 \bar{B}(x,y)- \pi_1 \bar{B}(x,0), \quad \bar \pi_2(x,y)= \pi_2 \bar{B}(x,y)- \pi_2 \bar{B}(x,0),$$
are functions whose norms are $O(\delta^2)$.

\subsection{Defining renormalization: critical projection} 
 By the Argument Principle, 
if $\delta$ is sufficiently small, then 
%functions $\eta_1$, $\eta_2$, $\xi_1$ and $\xi_2$ have unique quadratic critical points in a small neighborhood of $0$ in $\CC$. In particular, 
the function $\pi_1 \bar B \circ \bar A (x,0)$ has a unique critical point $c_1$ in a neighborhood of $0$. Set $T_1(x,y)=(x+c_1,y)$, then
$$\partial_x \left(\pi_1 T_1^{-1} \circ \bar B \circ \bar A \circ T_1  \right)(0,0)=0.$$ Similarly, if $\delta$ is sufficiently small, the function $\pi_1 T_1^{-1} \circ \bar A \circ \bar B \circ T_1(x,0)$ has a unique critical point $c_2$ in a neighborhood of $0$.  Set $T_2(x,y)=(x+c_2,y)$, then
$$\partial_x \left(\pi_1 T_2^{-1} \circ T_1^{-1} \circ \bar A \circ \bar B \circ T_1  \circ T_2 \right)(0,0)=0.$$

We now set
\begin{eqnarray}
\nonumber \Pi_1(\bar A, \bar B)&=&(\tilde A, \tilde B):=(T_2^{-1} \circ T_1^{-1} \circ \bar A \circ T_1, T^{-1}_1 \circ \bar B \circ T_1 \circ T_2)\\
\nonumber &=& \left( \left( \tilde \eta_1(x) + \tilde \tau_1(x,y) \atop   \tilde \eta_2(x) + \tilde \tau_2(x,y)  \right), \left( \tilde \xi_1(x) + \tilde \pi_1(x,y) \atop   \tilde \xi_2(x) + \tilde \pi_2(x,y)  \right)   \right),
\end{eqnarray}
where the norms of the functions $\tilde \tau_k$, $\tilde \pi_k$, $k=1,2$, are $O(\delta^2)$. 

The critical points  of the functions $\pi_1 (\bar A \circ \bar B)(x,0)$ and $\pi_1 (\bar B \circ \bar A)(x,0)$ are $O\left( \delta \|\pi_1 \Sigma -\pi_2 \Sigma \|  +\delta^{2} \right)$-close to each other, and therefore, 
\begin{equation}
\label{T2small} T_2=\text{Id}+O\left( \delta  \|\pi_1 \Sigma -\pi_2 \Sigma \|  +\delta^{2} \right).
\end{equation}

Let us set 
$$\tl\Sigma=(\tl A,\tl B)=\Pi_1 p \cR^n\Sigma.$$
We note that if the maps $\bar A$ and $\bar B$ commute, than the critical point of $\pi_1 T_1^{-1} \circ \bar A \circ \bar B \circ T_1(x,0)$ is at $0$. We, therefore, have the following
\begin{prop}
Suppose $(A,B)$ is a pre-renormalization of a map $H$. Then the map $T_2\equiv \text{Id}$, and hence, the projection $\Pi_1$ is a conjugacy by $T_1$.
\end{prop}


\subsection{Defining renormalization: commutation projection} At the next step we will project the pair $(\tilde A, \tilde B)$ onto the subset of pairs satisfying the following almost commutation conditions:
\begin{eqnarray} \label{commutation}
\partial_x^i \pi_1(\tilde A \circ \tilde B(x,0) - \tilde B \circ \tilde A(x,0))\arrowvert_{x=0}&=&0, \quad i=0,2 \\
\label{normalization} \pi_1 \tilde B(0,0)&=&1.
\end{eqnarray}
To that end we set 
$$\Pi_2 (\tilde A,\tilde B)(x,y)=\left( \left( \tilde \eta_1(x) +a x^4+b x^6 + \tilde \tau_1(x,y) \atop   \tilde \eta_2(x) +a x^4+b x^6+ \tilde \tau_2(x,y)  \right), \left( \tilde \xi_1(x)+c  + \tilde \pi_1(x,y) \atop   \tilde \xi_2(x) +c +\tilde \pi_2(x,y)  \right)   \right),$$
and require that $(\ref{commutation})$ and $(\ref{normalization})$ are satisfied for maps in the pair $\Pi_2 (\tilde A,\tilde B)(x,y)$. The following Proposition is proved in \cite{GaYa2}.
\begin{prop}\label{prop:2Dprojection}
There exists $\rho>0$ such that for all $\tl\Sigma$ in the $\rho$-neighborhood of $$\iota(\cC(\alpha_n(\hat Z),\alpha_n(\hat W)))$$
there is a unique tuple $(a,b,c,d)$ such that the pair $ \Pi_2 (\tilde A,\tilde B)$ satisfies the equations $(\ref{commutation})$ and $(\ref{normalization})$. Moreover, in this neighborhood, the dependence of $\Pi_2$ on $\Sigma$ is analytic.  
Furthermore, if $A\circ B=B\circ A$, then 
$\Pi_2=\text{Id}.$

%Finally, if $$\Sigma=\left( \zeta \atop \zeta \right) \equiv \left(\left(\eta \atop \eta  \right), \left(\xi \atop \xi  \right)  \right) \in \iota(\cM(U,V)), $$ then 
%$$\Pi_2 (\tl A,\tl B)=\left(\cP \zeta \atop \cP \zeta  \right),$$
%where $\cP$ has been defined in (\ref{Pproj}). 
\end{prop}

\noindent
Let us fix $n\in 2\NN$, $\cU$, $Q$, $\delta$ so that Lemma~\ref{lem-preren}  holds, and furthermore, the image 
$\Pi_1p\cR^n\cA(\cU,Q,\delta)$ lies in the $\rho$-neighborhood of $\iota(\cC(\alpha_n(\hat Z),\alpha_n(\hat W)))$ as in Proposition~\ref{prop:2Dprojection}. We then have:

\begin{prop}
\label{small-pert2}
For every $\Sigma \in \cA(\cU,Q,\delta)$,
$${\rm dist}(\Pi_2\Pi_1 p \cR^n \Sigma, \iota(\cB(\alpha_n(\hat Z),\alpha_n(\hat W)))) < {C { \delta (\|  \pi_1 \Sigma-\pi_2 \Sigma\|+\delta   )}}.$$
\end{prop}


Let $\ell_n=\pi_1\bar B(0,0)$ and  $\Lambda_n(x,y)=(\ell_n x, \ell_n y)$.
\begin{defn}
 We define {\it the  renormalization of depth $n$ } of a pair $\Sigma \in \cA(\cU,Q,\delta)$ as
\begin{equation}\label{2Drenorm}
\cR_n\Sigma = \Lambda_n^{-1} \circ\Pi_2\circ\Pi_1\circ p\cR^n \Sigma \circ \Lambda_n.
\end{equation}
Given a map  $H$ from a subset of $\CC^2$ to $\CC^2$, such that the pair $(A,B)=p\cR^nH=(H^{q_{n+1}},H^{q_n}) \in  \cA(\cU,Q,\delta)$ for some integer $n$, we will also use the shorthand notation 
\[
\cR_n H \equiv \Lambda_n^{-1} \circ\Pi_2\circ\Pi_1\circ p\cR^n H \circ \Lambda_n.
\]
\end{defn}

\subsection{Hyperbolicity of renormalization of 2D dissipative maps}
%Let $n$ be an even number as above. 
We conclude this section by formulating the following theorem:
\begin{thm}
\label{mainthm6}
Given a $p$-periodic $\theta$, set that $\lambda=e^{2 \pi i\theta}$. Assume that {\rm ({\bf H})} holds.  Then there exists an even $n=m k$, where $m \in \NN$ and $k$ is as in $(\ref{k-def})$, such that the point $\iota(\zeta_\lambda)$ is a fixed point of $\cR_n$ in $O(\Omega,\Gamma)$. The linear operator
$N=D \cR_n \arrowvert_{\iota(\zeta_\lambda)}$  is compact. The spectrum of $N$ coincides with the spectrum of $M$, where $M$ is as in {\rm ({\bf H})}. More specifically, $\kappa \neq 0$ is an eigenvalue of $M$, and $h$ is a corresponding eigenvector if and only if $\kappa$ is an eigenvalue of $N$, and $D\iota(h)$ is a corresponding eigenvector.
\end{thm}
\begin{proof}
Since $\iota$ is an immersion on $\cC(Z,W)$, and 
$$\iota\circ \cR^k=\cR_k\circ\iota, $$
the spectral decomposition of $N$ splits into the direct sum $T_1\oplus T_2$, where $T_1$ is the tangent subspace
$$T_1=T_{\iota(\zeta_\lambda)}\iota(\cB(Z,W)).$$
The restriction $N|_{T_1}$ is isomorphic to $M$. Further, by 
Proposition~\ref{small-pert2}, the magnitude of a perturbation of $\iota(\zeta_\lambda)$ in the direction of a vector in $T_2$ is decreased quadratically by 
$(\cR_n)^2$. Hence, in the spectral decomposition, the subspace $T_2$ corresponds to the zero eigenvalue.
\end{proof}


